Reliable Gradient-free and Likelihood-free Prompt Tuning

Due to privacy or commercial constraints, large pre-trained language models (PLMs) are often offered as black-box APIs. Fine-tuning such models to downstream tasks is challenging because one can neither access the model's internal representations nor propagate gradients through it. This paper addresses these challenges by developing techniques for adapting PLMs with only API access. Building on recent work on soft prompt tuning, we develop methods to tune the soft prompts without requiring gradient computation. Further, we develop extensions that in addition to not requiring gradients also do not need to access any internal representation of the PLM beyond the input embeddings. Moreover, instead of learning a single prompt, our methods learn a distribution over prompts allowing us to quantify predictive uncertainty. Ours is the first work to consider uncertainty in prompts when only having API access to the PLM. Finally, through extensive experiments, we carefully vet the proposed methods and find them competitive with (and sometimes even improving on) gradient-based approaches with full access to the PLM.

==> Sections/Rebuttal.tex <==
\section{Rebuttal}
\subsection{Reviewer wTbA}
\paragraph{(1) Regarding the empirical gain.}
The empirical gain on the uncertainty quantification tasks is non-trivial as measured by the AURRRC score. The "Performance Metrics" segment in Section 5.1 discuss that the AURRRC measures the area under risk vs. rejection rate curve, i.e., the portion of incorrectly predicted samples or portion of OOD samples after the model abstained some samples based on uncertainty measurement. Note that an oracle with perfect knowledge of uncertainty measurement can achieve a minimum AURRRC score. This is obtained by assigning an uncertainty score based on the oracle knowledge, i.e., whether a test sample is incorrectly predicted (OOD data or not). We measure such minimum AURRRC score as the performance lower-bound. Specifically, take the OOD detection task as an example. Suppose the test samples consist of N in-distribution samples and N OOD samples. We assign small uncertainty scores, such as 0, to all in-distribution samples and assign large uncertainty scores, such as 100, to all OOD samples. Then at rejection rate $20\%$, the corresponding risk value is $\frac{0.6N}{1.6N}=0.375$. After averaging the risk value corresponding to all possible rejection rates, we will obtain the minimum possible AURRRC score. As shown in Tables 1-3, our proposed method improves the average AURRRC score over the baseline(BBT) by $24.1\%$ on the selective classification task,  $15\%$ on the far OOD detection task, and $7\%$ on near OOD detection task, thereby demonstrating a significant improvement.
\begin{table*}[!t]
  \begin{center}
  \tiny
  \caption{\textbf{Selective Classification} (AURRRC score $\boldsymbol{\downarrow}$)}
  \vspace{-1.5em}
  \begin{tabular}{llllllllll}
    \\
    \toprule
    \textbf{Settings} & \textbf{Methods} & \textbf{SST-2} & \textbf{Yelp P.}& \textbf{AG’s News} & \textbf{DBPedia}& \textbf{MRPC} &\textbf{SNLI} &\textbf{RTE} &\textbf{Avg}\\
    \hline
    & \textbf{Lower-bound} & 0.030 & 0.009 &  0.035 & 0.070 & 0.251 & 0.427 & 0.255 & 0.154  \\
    \hline
    Gradient-free& BBT(Entropy) & 0.063$\pm$0.009 & 0.029$\pm$0.001 & 0.082$\pm$0.004 & 0.095$\pm$0.009 & 0.349$\pm$0.002 & 0.519$\pm$0.032 & 0.523$\pm$0.004 & 0.237  \\
    & BBT(MaxP) & 0.063$\pm$0.009 & 0.029$\pm$0.001 & 0.077$\pm$0.004 & 0.091$\pm$0.009 & 0.349$\pm$0.002 & 0.513$\pm$0.031 & 0.523$\pm$0.004 & 0.235  \\
              & \textbf{Ours(ELBO)(Entropy)} & 0.053$\pm$0.004 & 0.026$\pm$0.001 & 0.079$\pm$0.001 & 0.123$\pm$0.006 & 0.336$\pm$0.009 & 0.481$\pm$0.065 & 0.508$\pm$0.012 & 0.229\\
              & \textbf{Ours(ELBO)(MaxP)} & 0.053$\pm$0.004 & 0.026$\pm$0.001 & 0.074$\pm$0.002 & 0.117$\pm$0.005 & 0.336$\pm$0.009 & 0.478$\pm$0.062 & 0.508$\pm$0.012 & 0.227\\
              & \textbf{Ours(Ensembles)(Entropy)}     & 0.046$\pm$0.006 & 0.023$\pm$0.001 & 0.074$\pm$0.002 & 0.084$\pm$0.004 & 0.324$\pm$0.011 & 0.472$\pm$0.048 & 0.513$\pm$0.048 & 0.219\\
              & \textbf{Ours(Ensembles)(MaxP)}     & 0.046$\pm$0.006 & 0.023$\pm$0.001 & 0.068$\pm$0.002 & 0.076$\pm$0.004 & 0.324$\pm$0.011 & 0.469$\pm$0.047 & 0.513$\pm$0.048 & \textbf{0.217}\\
    \toprule
  \end{tabular}
  \label{table:selective-lowerbound}
  \end{center}
   \vspace{-1em}
\end{table*}

\begin{table*}[h]
  \begin{center}
  \tiny
  \caption{\textbf{Far OOD Detection} (AURRRC score $\boldsymbol{\downarrow}$)}
  \vspace{-1.5em}
  \begin{tabular}{llllllllll}
    \\
    \toprule
    \textbf{Settings} & \textbf{Methods} & \makecell[l]{ID:\textbf{SST-2}\\ OOD:\textbf{RTE}} & \makecell[l]{ID:\textbf{Yelp P.}\\ OOD:\textbf{RTE}} &\makecell[l]{ID:\textbf{MRPC}\\ 
    OOD:\textbf{RTE}}&  \makecell[l]{ID:\textbf{DBPedia}\\ OOD:\textbf{AG’s News}}
    &\makecell[l]{ID:\textbf{SNLI}\\ OOD:\textbf{MRPC}}& \makecell[l]{ID:\textbf{RTE}\\ OOD:\textbf{MRPC}} &\textbf{Avg}\\
    \hline
    & \textbf{Lower-bound} & 0.072 & 0.001 & 0.162 & 0.010 & 0.004 & 0.357 & 0.101   \\
    \hline
    Gradient-free& BBT(entropy) & 0.124$\pm$0.015 & 0.002$\pm$0.000 & 0.404$\pm$0.006 & 0.058$\pm$0.018 & 0.100$\pm$0.002 & 0.639$\pm$0.024 &0.221 \\
             & BBT(MaxP) & 0.124$\pm$0.015 & 0.002$\pm$0.000 & 0.404$\pm$0.006& 0.059$\pm$0.014 & 0.098$\pm$0.002 & 0.639$\pm$0.024 &0.221 \\
              & \textbf{Ours(ELBO)(Entropy)} & 0.112$\pm$0.010 & 0.001$\pm$0.000 & 0.320$\pm$0.014 & 0.051$\pm$0.001 & 0.109$\pm$0.002 & 0.635$\pm$0.003 &0.205 \\
              & \textbf{Ours(ELBO)(MaxP)} & 0.112$\pm$0.010 & 0.001$\pm$0.000 & 0.320$\pm$0.014 & 0.056$\pm$0.001 & 0.107$\pm$0.002 & 0.635$\pm$0.003 &0.205 \\
              & \textbf{Ours(Ensembles)(Entropy)}     & 0.097$\pm$0.008 & 0.001$\pm$0.000 & 0.350$\pm$0.038 & 0.057$\pm$0.003 & 0.110$\pm$0.001  & 0.606$\pm$0.047& 0.204 \\
              & \textbf{Ours(Ensembles)(MaxP)}   & 0.097$\pm$0.008 & 0.001$\pm$0.000 & 0.350$\pm$0.038 & 0.058$\pm$0.002 & 0.108$\pm$0.001  & 0.606$\pm$0.047& \textbf{0.203} \\
    \toprule
  \end{tabular}
  \label{table:far-OOD-detection-lowerbound}
  \end{center}
   \vspace{-1em}
\end{table*}

\begin{table*}[h]
  \begin{center}
  \tiny
  \caption{\textbf{Near OOD Detection} (AURRRC score $\boldsymbol{\downarrow}$)}
  \vspace{-1.5em}
  \begin{tabular}{llllllll}
    \\
    \toprule
    \textbf{Settings} & \textbf{Methods} & \makecell[l]{ID:\textbf{SST-2}\\ OOD:\textbf{IMDB}} & \makecell[l]{ID:\textbf{Yelp P.}\\ OOD:\textbf{IMDB}} &\makecell[l]{ID:\textbf{SNLI}\\ OOD:\textbf{MNLI}}& \makecell[l]{ID:\textbf{RTE}\\ OOD:\textbf{MNLI}} &\textbf{Avg}\\
    \hline
    & \textbf{Lower-bound} &  0.960 &  0.147 & 0.259 & 0.950 & 0.579    \\
    \hline
    Gradient-free & BBT(entropy) & 0.978$\pm$0.003 & 0.315$\pm$0.003 & 0.720$\pm$0.011 & 0.963$\pm$0.008 & 0.744  \\
              & BBT(confidence) & 0.978$\pm$0.003 & 0.315$\pm$0.003 & 0.705$\pm$0.011 & 0.963$\pm$0.008 & 0.740  \\
              & \textbf{Ours(ELBO)(Entropy)} & 0.976$\pm$0.002 & 0.308$\pm$0.006 & 0.692$\pm$0.039 & 0.968$\pm$0.005 & 0.736  \\
              & \textbf{Ours(ELBO)(MaxP)} & 0.976$\pm$0.002 & 0.308$\pm$0.006 & 0.678$\pm$0.044 & 0.968$\pm$0.005 & 0.733  \\
              & \textbf{Ours(Ensembles)(Entropy)}     & 0.976$\pm$0.001 & 0.297$\pm$0.003 & 0.707$\pm$0.028 &  0.962$\pm$0.002 & 0.736 \\
              & \textbf{Ours(Ensembles)(MaxP)}     & 0.976$\pm$0.001 & 0.297$\pm$0.003 & 0.692$\pm$0.032 & 0.962$\pm$0.002 & \textbf{0.732} \\
    \toprule
  \end{tabular}
  \label{table:near-OOD-detection-lowerbound}
  \end{center}
   \vspace{-1em}
\end{table*}








\paragraph{(2) "Why are logits and likelihood used interchangeably in the paper?"}
We were not implying "logits" and "likelihood" are equivalent, but that in the classification setting considered in this paper, likelihood computation requires access to the logits. We use the terms likelihood and likelihood-free to describe the problem setting --- whether or not we can compute the likelihood during optimization. By "logits" we denote the output of a pretrained language model(PLM), i.e., whether the raw outputs from PLM are the logits or the discrete outcome labels. We will clarify this further in the paper. 

%We only use the terms interchangeably to describe the "likelihood-free" setting because, in practice, without accessing logits implies that likelihood is also not available. 

\paragraph{(3) Regarding the notation of $f$.}
We agree with the reviewer that using a single notation $f$ to denote the pre-trained language model(PLM) could be an abuse of notation, as the outputs of $f$ can be different under different contexts and problem settings. In general, the output of $f$ under the likelihood setting is a label distribution but a discrete token under the likelihood-free setting. Although we provide a sufficient explanation (in words), we will use different notations in the revised version to make it easier to distinguish different settings.

\paragraph{(4) Regarding the limitation of CMA-ES Algorithm.}
% CMA-ES Algorithm indeed has the issue, as the reviewer pointed out, but we empirically observe that it achieves good performance, and we provide our intuitive justification as follows. Gradient-free prompt tuning is equivalent to optimizing a small portion of the parameter (the soft prompts) of an over-parameterized pre-trained language model(PLM) w.r.t. specific objective function using the CMA-ES optimizer. It is well known that an over-parameterized model trained using SGD also has the "local minimum" or "bad initialization" issue. However, people discover that such a "sub-optimal" model can still empirically perform well [1]. Thus, we conjecture that as we optimize the soft prompts conditioned on the over-parameterized PLM, the existing explanation of the "local minimum" issue of PLM might also be valid. 

CMA-ES Algorithm may have "bad initialization" and "local minima" issues, as pointed out by the reviewer. However, we empirically observe that it achieves good performance, and we believe that over-parameterization might be the reason. It is well-known that a pre-trained language model (PLM) is usually trained using SGD, which also has the "local minima" or "bad initialization" issue. However, recent progress in learning theory has shown that SGD can find good local minima in an over-parameterized model, and this explains the empirical success of local optimization algorithms like SGD [1,2]. Gradient-free prompt tuning is equivalent to optimizing a small fraction of the parameters (the soft prompts) of an over-parameterized PLM w.r.t. specific objective function using the CMA-ES optimizer. Thus, we conjecture that as we optimize the soft prompts conditioned on the over-parameterized PLM, the same explanation of the "local minima" issue with SGD might also be valid in our setting. 

As for the "large iteration" issue, though a longer training time is required compared to the gradient-based approach, the actual training time is still reasonable, and it is the price we need to pay for the gradient-free constraint. As elaborated in the "implementation details" section of the Appendix, the maximum number of iterations required for the CMA-ES algorithm is 300 in practice. Hence, it requires less than 24h of training on a single device for any dataset we evaluated in this work.

[1] Deep Learning without Poor Local Minima, NIPS 2016.

[2] A Convergence Theory for Deep Learning via Over-Parameterization, ICML 2019.

\paragraph{(5) "How is the running time of the sequential Monte Carlo methods based SBI?"}
We report the training time of our proposed SBI approach on all benchmark datasets and compare it with the training time of the gradient-free baseline method BBT as follows. Though the ABC-SMC approach takes longer training time than BBT on some challenging benchmark datasets, the training time is still in a reasonable range. In general, the training time on a single device for any dataset is within 24 hours, and the longer training time is the price we have to pay for the much more strict likelihood-free constraint.

\begin{table*}[h]
  \begin{center}
  \tiny
  \caption{\textbf{Training Time} (Runtime in seconds)}
  \vspace{-1.5em}
  \begin{tabular}{llllllllll}
    \\
    \toprule
    \textbf{Settings} & \textbf{Methods} & \textbf{SST-2} & \textbf{Yelp P.}& \textbf{AG’s News} & \textbf{DBPedia}& \textbf{MRPC} &\textbf{SNLI} &\textbf{RTE} &\textbf{Avg}\\
    \hline
    Gradient-free & BBT & 1034.7 s & 3636.5 s & 2988.4 s & 3739.4 s & 1597.9 s & 1541.7 s & 2552.5 s & 2441.6 s  \\\hline
    \makecell{Likelihood-free} & \textbf{Ours(ABC-SMC)} & 1331.3 s & 1839.9 s & 37574.1 s & 75927.8 s & 1801.7 s & 30393.5 s & 66155.9 s & 30717.7 s\\
    \toprule
  \end{tabular}
  \label{table:runtime}
  \end{center}
   \vspace{-1em}
\end{table*}

\subsection{Reviewer Miz3 }
\paragraph{(1) Regarding the technical novelty of this work.}
% The main novelty of this work includes: (1)Addressing a novel prompt tuning problem that has never been considered in the literature, i.e., the likelihood-free setting. (2)As far as we know, no one has considered the Bayesian framework or proposed Bayesian approaches for prompt tuning under gradient-free and likelihood-free settings. The contribution of this work is to adapt the Bayesian approaches, such as variational inference, to achieve uncertainty quantification for prompt tuning. The CMA-ES algorithm simply serves as an optimizer as the surrogate of SGD under the gradient-free setting.

% Thus, the scope of this work is to discover and formulate a novel and important problem with practical benefits and propose efficient techniques to tackle it. Proposing new derivative-free optimization algorithms or SBI algorithms is out of the scope of this work and should be considered as another research problem orthogonal to prompt tuning.

The main novelty of this work includes: (1) Addressing a novel prompt tuning problem that has never been studied in the literature, i.e., the likelihood-free setting. (2)Resolving prompt tuning problems under gradient-free and likelihood-free settings using the proposed Bayesian approaches to improve uncertainty quantification performance. As far as we know, no one has considered the Bayesian framework for prompt tuning under gradient-free and likelihood-free settings. Thus, the scope of this work is to discover and formulate a novel problem with practical significance and propose efficient techniques to tackle it.

The CMA-ES algorithm simply serves as an optimizer as the surrogate of SGD under the gradient-free setting. Constructing new derivative-free optimization algorithms or SBI algorithms is out of the scope of this work and should be considered as a separate research problem. % orthogonal to prompt tuning.

\paragraph{(2) Regarding the calibration performance on AG's News dataset.}
A possible explanation of the reported sub-optimal calibration performance on AG's News dataset is that the Bayesian approach gives a less confident predictive distribution. First, the class number of AG's News dataset is larger than other tasks. Second, we use relatively small prompt samples to estimate the predictive label distribution to ensure efficient inference, which might lead to less concentrated label distribution and a relatively large ECE error. Even if the prediction lacks sufficient confidence, it is still beneficial for the downstream uncertainty quantification tasks, such as selective classification, since it can prevent over-confident prediction on those wrong-predicted samples. In practice, good calibration performance is usually sufficient but not necessary for the model to perform well on the downstream uncertainty quantification tasks.

\subsection{Reviewer mKQV}
\paragraph{(1) Regarding the training complexity of SBI.}


\paragraph{(2) Regarding more discussion about related literature.}
We have included some discussion about uncertainty quantification for NLP in "Beyond point-estimates of prompts" in Section 2. As suggested by the reviewer, we will add more detailed discussions and introduce more relevant literature in the revised version.

\subsection{Reviewer 8QNX}
We thank the reviewer for the detailed feedback and valuable suggestions. We hope the following response resolves the major concerns.
\paragraph{(1) Regarding Notations}
We use $\mathcal{D}$ with calligraphic font type to denote the "dataset" and use $D$ with default font type to denote the "dimension". We acknowledge the reviewer's concern regarding the notations, we will re-visit all of them and elaborate on some of the notations so as to better the readability of the paper.

\paragraph{(2) Regarding soft prompt $\bm{z}$}
As we introduced in the background section, the soft prompt tuning (Li and Liang, 2021) aims to learn a continuous prompt $\mathbf{P}$ as the parameter (a continuous vector) injected into the embedding layer of pre-trained language model(PLM). In this work, we follow the soft prompt tuning setting of BBT (Sun et al., 2022b). Given that the details about soft prompt $\boldsymbol{z}$ are already discussed in the BBT paper, here we briefly recap it in the problem formulation section. Instead of a masking template or discrete text, $\boldsymbol{z}$ is the low-dimensional subspace representation of the continuous prompt $\mathbf{P}$. The pre-trained language model(PLM) take the concatenation of both the soft prompt $\mathbf{P}$ and the embedding of input text $\tilde{\mathbf{X}}$ as the inputs to make the prediction. We will add more clarification in the revised version.

==> Sections/With-likelihood.tex <==
\section{Likelihood Setting}
When the likelihood is available, i.e. the output logits of PTM are accessible, MCMC is the typical Monte Carlo approach to approximate the posterior distribution, but it usually suffers from the computational issue of low convergence. Alternatively, we consider two approaches commonly utilized as Bayesian inference techniques for modern neural networks, including variational inference and ensembles. However, both of these traditional inference algorithms require the model gradient to allow back-propagation, which is not applicable under the black-box setting. Since the CMA-ES algorithms is known to be super efficient for black-box optimization, we propose the gradient-free variational inference and ensembles algorithms with CMA-ES as an essential ingredient.

\subsection{Gradient-free Variational Inference} \label{sec: ELBO}
Since direct computation of prompt posterior distribution $P(\vz|\gD)$ is intractable, variational inference approximates the posterior distribution with a tractable distribution over the prompt embedding $q(\vz ; \boldsymbol{\lambda})$, where $\boldsymbol{\lambda}$ is the variational parameter as the target to optimize such that the KL-divergence between true posterior distribution and variational distribution is minimized, i.e., $\boldsymbol{\lambda}^{\star} = \argmin_{\boldsymbol{\lambda}} \mathrm{KL}\left(P(\vz|\gD) \|  q(\vz ; \boldsymbol{\lambda}) \right) $. Because the KL term cannot be evaluated directly, we instead maximize the evidence lower bound (ELBO), i.e., 
\begin{align} 
\boldsymbol{\lambda}^{\star} =& \argmax_{\boldsymbol{\lambda}} \; \mathbb{E}_{q(\vz ; \boldsymbol{\lambda})}[\log P(\gD|\vz) ]   \nonumber\\
&- \mathrm{KL}\left( q(\vz ; \boldsymbol{\lambda}) \| P(\vz) \right) \\
=& \argmax_{\boldsymbol{\lambda}} \; \sum_{i=1}^{n} \mathbb{E}_{q(\vz ; \boldsymbol{\lambda})}[\log  P(\tilde{y}_i|\tilde{\vx}_i; \vz) ]  \nonumber\\
&- \mathrm{KL}\left( q(\vz ; \boldsymbol{\lambda}) \| P(\vz) \right)
\label{eq:ELBO}
\end{align}
Optimizing the ELBO objective requires taking derivative w.r.t $\boldsymbol{\lambda}$. According to chain rule, this also requires the gradient of log likelihood w.r.t $\vz$, i.e., $\nabla_{\vz} \log  P(\tilde{y}_i|\tilde{\vx}_i; \vz)= \nabla_{\vz} \log f(\mathbf{A}\vz+\mathbf{P_0};\tilde{\vx}_i)$, which causes the variational inference training infeasible under the black-box setting.

Instead of gradient descent and back-propagation, we propose a gradient-free variational inference algorithm using the derivative-free optimizer CMA-ES. Unlike BBT \citep{sun2022black} uses CMA-ES to optimize the prompt embedding $\vz$ directly, we instead optimize the variational parameter $\boldsymbol{\lambda}$. We consider the variational distribution as a multivariate Normal distribution $q(\vz ; \boldsymbol{\lambda})= \gN(\boldsymbol{\mu},\boldsymbol{\Sigma})$, where we assume the covariance matrix is a diagonal matrix, i.e.,  $\boldsymbol{\Sigma}=\operatorname{diag}(\boldsymbol{\alpha}) \in \sR^{d\times d}$. Thus, the variational parameter is mean and diagonal elements of the covariance matrix, i.e., $\boldsymbol{\lambda} = (\boldsymbol{\mu},\boldsymbol{\alpha}) \in \sR^{2d}$. At each iteration of optimization, the CMA-ES algorithm outputs a collection of candidate solutions $\{\boldsymbol{\lambda}_j\}_{j=1}^m=\{ (\boldsymbol{\mu}_j,\boldsymbol{\alpha}_j) \}_{j=1}^m$ by sampling from another multivariate Normal distribution $\gN(m_t,\sigma^2_t C_t)$, where $m_t \in \sR^{d}$ is the current mean solution to the optimization, $\sigma_t >0$ is the current step size to update the solution, and $C_t \in \sR^{d\times d}$ is the current covariance matrix controls the shape of normal distribution. For each possible solution of variational parameter $\boldsymbol{\lambda}_j$, we can evaluate the corresponding ELBO loss using the variational distribution $q(\vz ; \boldsymbol{\lambda}_j) = \gN(\boldsymbol{\mu}_j,\boldsymbol{\Sigma}_j)$, where the expectation in Equation~\ref{eq:ELBO} is approximated by Monte-Carlo samples sampled from the variational distribution. Finally, the CMA-ES optimizer takes current collection of solutions of variational parameter $\{\boldsymbol{\lambda}_j\}_{j=1}^m$ and their corresponding ELBO loss, update $m_t$, $\sigma_t$ and $C_t$ for next iteration. 

\begin{comment}
The overall framework is shown in Algorithm~\ref{alg:ELBO}.
\begin{algorithm}[h]
\SetAlgoLined
    \algorithmicinput{PTM $f$,  CMA-ES optimizer $\operatorname{CMA}$, Total iterations T}

Initialize the collection of variational parameter $\boldsymbol{\lambda}_j)$, 

%and discriminators $\{\vd^{s_j}\}_{j=1}^{m}$

Initialize the pseudo-label $\tilde{y}_i^t$ for each target data $\vx_i^t$ by~\eqref{eq:pseudo-label} using pretrained models $\{\vh^{s_j}\}_{j=1}^{m}$ and domain weights $\vw_j$ \\
\For{$\tau = 1,2, \ldots, T$}
{   
    Update $\gD_l$ and $\gD_u$ by \eqref{eq:split}
    
    \For{$j = 1,2, \ldots, m$}
    {
    \tcp*[h]{Update each source model}
    
    Update discriminators ${\vd^{s_{j}^{(\tau)}}}$ by maximizing~\eqref{eq:adv}. 
    
    Update feature extractor ${\vf^{s_j^{(\tau)}}}$ by minimizing~\eqref{eq:loss}.
    }
    Update the pseudo-label $\tilde{y}_i^t$ using domain weights $\vw_j$ and updated models $\{{\vh^{s_j^{(\tau)}}}\}_{j=1}^{m}$ by~\eqref{eq:pseudo-label}.
}

    \algorithmicoutput{ Updated models $\{{\vh^{s_j^{(T)}}}\}_{j=1}^{m}$, domain weights $\vw_j$}

 \caption{Gradient-free variational Inference}\label{alg:ELBO}
\end{algorithm}
\end{comment}

\subsection{Ensembles}
In practice, the posterior predictive distribution $P(\tilde{y}|\tilde{\vx}; \gD)$ is approximated by finite number of Monte Carlo samples, as shown in Equation~\ref{eq:predictive}. In practice, evaluating one prompt sample requires the forward pass of the entire PTM, which is computational expensive especially for large language model. The more practical way to approximate the posterior predictive distribution is using a limited number of most representative prompt posterior samples corresponding to high-density regions of posterior distribution. Deep ensemble~\citep{lakshminarayanan2017simple} turns out to be one of the most reliable approaches that can achieve this goal, which the typical way is re-training the model with different initializations, and averaging the prediction results of all the models. Again, although it is possible to train the prompt embedding in the same manner, it still requires accessing the gradient of PTM for back-propagation. To this end, we propose an simple but effective ensemble approach based on CMA-ES algorithm.

The CMA-ES algorithm requires a normal distribution $\gN(m_t,\sigma^2_t C_t)$ to sample a collection of samples. Our simple ensemble approaches is iterating CMA-ES algorithm for $K$ times with different random initialization of the mean $m_t$ and variance $\sigma$. After each iteration, we will obtain $\vz_k$ as an optimal prompt embedding. The collection of prompt embedding $\{\vz_k\}_{k=1}^K$ are the Monte Carlo samples used to approximate the label distribution.

